A Survey of Cybersecurity of Digital Manufacturing

The Industry 4.0 concept promotes a digital manufacturing (DM) paradigm that can enhance quality and productivity, that reduces inventory and the lead-time for delivering custom, batch-of-one products based on achieving convergence of Additive, Subtractive, and Hybrid manufacturing machines, Automation and Robotic Systems, Sensors, Computing, and Communication Networks, Artificial Intelligence, and Big Data. A DM system consists of embedded electronics, sensors, actuators, control software, and inter-connectivity to enable the machines and the components within them to exchange data with other machines, components therein, the plant operators, the inventory managers, and customers. This paper presents the cybersecurity risks in the emerging DM context, assesses the impact on manufacturing, and identifies approaches to secure DM.

==> table.tex <==
\begin{table*}[t!]
\centering
\begin{tiny}
\caption{Categorization of DM Security studies. ``DoS'', ``Rev. Engg.'', ``Tamper'', ``Unreliable'', Cov. channel'' stand for ``Denial of Service'', ``Reverse Engineering'', ``Tampering data'', ``Reduce reliability'', and ``covert channel'', respectively. \textcolor{red}{Red rows are attack case studies in section \ref{sec:threats}}. \textcolor{blue}{Blue rows are defense case studies in section \ref{sec:defense}}.}
\label{tab:summary}
\resizebox{0.935\textwidth}{!}{%
\begin{tabular}{|lccccccccccccc|}
\specialrule{1pt}{1pt}{1pt}
 & \multicolumn{2}{c|}{\textbf{}} & \multicolumn{3}{c|}{\textbf{Attack Goals}} & \multicolumn{7}{c|}{\textbf{Attacks}} \\
\textbf{Papers} & \rotatebox{90}{Attacks} & \multicolumn{1}{c|}{\rotatebox{90}{Defenses}} & {\rotatebox{90}{Piracy}} & \rotatebox{90}{Sabotage} & \multicolumn{1}{c|}{\rotatebox{90}{Counterfeit}} & {\rotatebox{90}{DoS}} & {\rotatebox{90}{Rev. Engg.}} & {\rotatebox{90}{Tamper}} & \rotatebox{90}{Unreliable} & \rotatebox{90}{Sidechannel} & \rotatebox{90}{Cov.channel} & \multicolumn{1}{c|}{\rotatebox{90}{IP Theft}}\\ \specialrule{0.8pt}{1pt}{1pt}
\rowcolor[HTML]{DFDFDF} 
Gupta \textit{et al.}~\cite{gupta2020additive} & & \multicolumn{1}{c|}{\checkmark} &  & \checkmark & \multicolumn{1}{c|}{} & & & \checkmark & & & & \multicolumn{1}{c|}{\checkmark}\\
Strurm \textit{et al.}~\cite{sturm2017cyber} & & \multicolumn{1}{c|}{} &  & \checkmark & \multicolumn{1}{c|}{\checkmark} & & & \checkmark & & & & \multicolumn{1}{c|}{}\\
\rowcolor[HTML]{DFDFDF} 
Ranabhat \textit{et al.}~\cite{ranabhat2019optimal} & \checkmark & \multicolumn{1}{c|}{} &  & \checkmark & \multicolumn{1}{c|}{} & & & \checkmark & \checkmark & & & \multicolumn{1}{c|}{}\\
\textcolor{red}{Belikovetsky \textit{et al.}~\cite{belikovetsky2017dr0wned}} & \textcolor{red}{\checkmark} & \multicolumn{1}{c|}{} &  & \textcolor{red}{\checkmark} & \multicolumn{1}{c|}{\textcolor{red}{\checkmark}} & & \textcolor{red}{\checkmark} &  & & & \textcolor{red}{\checkmark} & \multicolumn{1}{c|}{}\\
\rowcolor[HTML]{DFDFDF} 
Yampolskiy \textit{et al.}~\cite{yampolskiy2016using} & & \multicolumn{1}{c|}{\checkmark} &  & \checkmark & \multicolumn{1}{c|}{} & & & & \checkmark & & & \multicolumn{1}{c|}{}\\
Wu \textit{et al.}~\cite{wu2019detecting} & & \multicolumn{1}{c|}{\checkmark} &  & \checkmark & \multicolumn{1}{c|}{} & & & \checkmark & & \checkmark & & \multicolumn{1}{c|}{\checkmark}\\
\rowcolor[HTML]{DFDFDF} 
Chhetri \textit{et al.}~\cite{chhetri2016kcad} & & \multicolumn{1}{c|}{\checkmark} &  & \checkmark & \multicolumn{1}{c|}{} & & & \checkmark & \checkmark & \checkmark & & \multicolumn{1}{c|}{}\\
Desmit \textit{et al.}~\cite{desmit2016cyber} & \checkmark & \multicolumn{1}{c|}{} & \checkmark &  & \multicolumn{1}{c|}{} & & & \checkmark & \checkmark & & & \multicolumn{1}{c|}{\checkmark}\\
\rowcolor[HTML]{DFDFDF} 
Chen \textit{et al.}~\cite{chen2017security} & & \multicolumn{1}{c|}{\checkmark} &  & \checkmark & \multicolumn{1}{c|}{\checkmark} & & & & & & & \multicolumn{1}{c|}{\checkmark}\\
Elhabashya \textit{et al.}~\cite{elhabashya2019cyber} & & \multicolumn{1}{c|}{\checkmark} &  & \checkmark & \multicolumn{1}{c|}{} & & & \checkmark &  & \checkmark & & \multicolumn{1}{c|}{\checkmark}\\
\rowcolor[HTML]{DFDFDF} 
\textcolor{red}{Moore \textit{et al.}~\cite{moore2017implications}} & \textcolor{red}{\checkmark} & \multicolumn{1}{c|}{} &  & \textcolor{red}{\checkmark} & \multicolumn{1}{c|}{} & \textcolor{red}{\checkmark}  & & \textcolor{red}{\checkmark} & \textcolor{red}{\checkmark} & & & \multicolumn{1}{c|}{}\\
Bracho \textit{et al.}~\cite{bracho2018simulation} & & \multicolumn{1}{c|}{\checkmark} &  &  & \multicolumn{1}{c|}{} & & &  & & \checkmark & \checkmark & \multicolumn{1}{c|}{\checkmark}\\
\rowcolor[HTML]{DFDFDF} 
Graves \textit{et al.}~\cite{graves2019characteristic} & \checkmark & \multicolumn{1}{c|}{} & \checkmark & \checkmark & \multicolumn{1}{c|}{} & & & & & & & \multicolumn{1}{c|}{\checkmark}\\
Yampolskiy \textit{et al.}~\cite{yampolskiy2014intellectual} & & \multicolumn{1}{c|}{\checkmark} & \checkmark &  & \multicolumn{1}{c|}{} & & \checkmark & \checkmark & & \checkmark & & \multicolumn{1}{c|}{\checkmark}\\
\rowcolor[HTML]{DFDFDF} 
Chhetri \textit{et al.}~\cite{chhetri2017security} & & \multicolumn{1}{c|}{\checkmark} &  &  & \multicolumn{1}{c|}{} & & \checkmark & \checkmark & & \checkmark & & \multicolumn{1}{c|}{\checkmark}\\
Belikovetsky \textit{et al.}~\cite{belikovetsky2017detecting} & & \multicolumn{1}{c|}{\checkmark} & \checkmark & \checkmark & \multicolumn{1}{c|}{} & & & \checkmark & & \checkmark & & \multicolumn{1}{c|}{}\\
\rowcolor[HTML]{DFDFDF} 
Chhetri \textit{et al.}~\cite{chhetri2017side} & & \multicolumn{1}{c|}{\checkmark} &  &  & \multicolumn{1}{c|}{} & & \checkmark &  & & \checkmark &  & \multicolumn{1}{c|}{\checkmark}\\
Baumann \textit{et al.}~\cite{baumann2017additive} & & \multicolumn{1}{c|}{\checkmark} &  &  & \multicolumn{1}{c|}{} & & \checkmark & \checkmark & & & & \multicolumn{1}{c|}{\checkmark}\\
\rowcolor[HTML]{DFDFDF} 
Wu \textit{et al.}~\cite{wu2018cybersecurity} & \checkmark & \multicolumn{1}{c|}{} &  & \checkmark & \multicolumn{1}{c|}{} & \checkmark & & \checkmark & & & & \multicolumn{1}{c|}{\checkmark}\\
\textcolor{blue}{Gupta \textit{et al.}~\cite{gupta2017obfuscade}} & \textcolor{red}{\checkmark} &  \multicolumn{1}{c|}{\textcolor{blue}{\checkmark}} &  & \textcolor{blue}{\checkmark} & \multicolumn{1}{c|}{\textcolor{blue}{\checkmark}} & & & \textcolor{red}{\checkmark} & & & & \multicolumn{1}{c|}{\textcolor{blue}{\checkmark}}\\
\rowcolor[HTML]{DFDFDF} 
Moore \textit{et al.}~\cite{moore2017power} & \checkmark & \multicolumn{1}{c|}{} & \checkmark & \checkmark & \multicolumn{1}{c|}{} & & &  & & \checkmark &  & \multicolumn{1}{c|}{\checkmark}\\
Tsoutsos \textit{et al.}~\cite{tsoutsos2017secure} &  &  \multicolumn{1}{c|}{\checkmark} &  &  & \multicolumn{1}{c|}{} & &  \checkmark & \checkmark & & & & \multicolumn{1}{c|}{}\\
\rowcolor[HTML]{DFDFDF} 
Belikovetsky \textit{et al.}~\cite{belikovetsky2018digital} & \checkmark & \multicolumn{1}{c|}{} &  & \checkmark & \multicolumn{1}{c|}{} & & \checkmark & \checkmark & \checkmark & \checkmark & & \multicolumn{1}{c|}{\checkmark}\\
Zarreh \textit{et al.}~\cite{zarreh2018cybersecurity} & & \multicolumn{1}{c|}{\checkmark} &  & \checkmark & \multicolumn{1}{c|}{} & \checkmark & & \checkmark & \checkmark & & & \multicolumn{1}{c|}{\checkmark}\\
\rowcolor[HTML]{DFDFDF} 
Miller \textit{et al.}~\cite{miller2018identifying} & & \multicolumn{1}{c|}{\checkmark} &  & & \multicolumn{1}{c|}{} &  & \checkmark & & & \checkmark & \checkmark & \multicolumn{1}{c|}{\checkmark}\\
Chaduvula \textit{et al.}~\cite{chaduvula2018security} &  & \multicolumn{1}{c|}{\checkmark} &  & \checkmark & \multicolumn{1}{c|}{\checkmark} & & & \checkmark & & & & \multicolumn{1}{c|}{}\\
\rowcolor[HTML]{DFDFDF} 
Raban \textit{et al.}~\cite{raban2018foresight} & \checkmark & \multicolumn{1}{c|}{\checkmark} &  & & \multicolumn{1}{c|}{\checkmark} &  & & \checkmark & & & \checkmark & \multicolumn{1}{c|}{\checkmark}\\
\textcolor{blue}{Chen \textit{et al.}~\cite{chen2019embedding}} &  & \multicolumn{1}{c|}{\textcolor{blue}{\checkmark}} &  & & \multicolumn{1}{c|}{\textcolor{blue}{\checkmark}} & & \textcolor{blue}{\checkmark} &  & & & & \multicolumn{1}{c|}{}\\
\rowcolor[HTML]{DFDFDF} 
Yu \textit{et al.}~\cite{yu2020sabotage} & & \multicolumn{1}{c|}{\checkmark} &  & \checkmark & \multicolumn{1}{c|}{} &  & & & & \checkmark & & \multicolumn{1}{c|}{}\\
Hoffman \textit{et al.}~\cite{hoffman2018internet} & & \multicolumn{1}{c|}{\checkmark} &  &  & \multicolumn{1}{c|}{} & & & \checkmark & \checkmark & & & \multicolumn{1}{c|}{\checkmark}\\
\rowcolor[HTML]{DFDFDF} 
Abdulhameed \textit{et al.}~\cite{abdulhameed2019additive} &  & \multicolumn{1}{c|}{\checkmark} &  & \checkmark & \multicolumn{1}{c|}{} &  & & \checkmark & & & & \multicolumn{1}{c|}{}\\
Padmanabhan \textit{et al.}~\cite{padmanabhan2018cybersecurity} & & \multicolumn{1}{c|}{\checkmark} &  & & \multicolumn{1}{c|}{} & & &  & \checkmark & & & \multicolumn{1}{c|}{\checkmark}\\
\rowcolor[HTML]{DFDFDF} 
Prinsloo \textit{et al.}~\cite{prinsloo2019review} &  & \multicolumn{1}{c|}{\checkmark} &  & \checkmark & \multicolumn{1}{c|}{} & \checkmark  & & \checkmark & & \checkmark & \checkmark & \multicolumn{1}{c|}{}\\
Chhetri \textit{et al.}~\cite{chhetri2019tool} & \checkmark & \multicolumn{1}{c|}{\checkmark} &  & & \multicolumn{1}{c|}{} & & &  & &  \checkmark & & \multicolumn{1}{c|}{}\\
\rowcolor[HTML]{DFDFDF} 
Calzado \textit{et al.}~\cite{jimenez2019additive} & & \multicolumn{1}{c|}{\checkmark} &  &  & \multicolumn{1}{c|}{} & & \checkmark & & & & & \multicolumn{1}{c|}{}\\
Yampolskiy \textit{et al.}~\cite{yampolskiy2015security} & \checkmark & \multicolumn{1}{c|}{} &  & \checkmark & \multicolumn{1}{c|}{} & & & \checkmark & & & & \multicolumn{1}{c|}{}\\
\rowcolor[HTML]{DFDFDF} 
Ivanova \textit{et al.}~\cite{ivanova2014unclonable} & & \multicolumn{1}{c|}{} &  &  & \multicolumn{1}{c|}{\checkmark} & & & \checkmark & & & & \multicolumn{1}{c|}{}\\
Bridges \textit{et al.}~\cite{bridges2015cyber} & & \multicolumn{1}{c|}{\checkmark} &  &  & \multicolumn{1}{c|}{} & & \checkmark & \checkmark & & \checkmark & & \multicolumn{1}{c|}{\checkmark}\\
\rowcolor[HTML]{DFDFDF} 
Holland \textit{et al.}~\cite{holland2017copyright} & & \multicolumn{1}{c|}{\checkmark} &  & & \multicolumn{1}{c|}{} & & & & & & & \multicolumn{1}{c|}{\checkmark}\\
Chhetri \textit{et al.}~\cite{chhetri2016poster} & \checkmark & \multicolumn{1}{c|}{} & \checkmark &  & \multicolumn{1}{c|}{} & & & & & \checkmark & & \multicolumn{1}{c|}{\checkmark}\\
\rowcolor[HTML]{DFDFDF} 
Wei \textit{et al.}~\cite{wei2018embedding} & & \multicolumn{1}{c|}{\checkmark} &  &  & \multicolumn{1}{c|}{\checkmark} & & \checkmark &  & & & & \multicolumn{1}{c|}{}\\
Wu \textit{et al.}~\cite{wu2017detecting} & & \multicolumn{1}{c|}{\checkmark} &  & \checkmark & \multicolumn{1}{c|}{} & & & \checkmark & & & & \multicolumn{1}{c|}{}\\
\rowcolor[HTML]{DFDFDF} 
Vincent \textit{et al.}~\cite{vincent2015trojan} & & \multicolumn{1}{c|}{\checkmark} &  & \checkmark & \multicolumn{1}{c|}{} & \checkmark & & & \checkmark & \checkmark & & \multicolumn{1}{c|}{\checkmark}\\
Riel \textit{et al.}~\cite{riel2017integrated} & & \multicolumn{1}{c|}{\checkmark} &  &  & \multicolumn{1}{c|}{} & \checkmark & &  & & \checkmark & \checkmark & \multicolumn{1}{c|}{}\\
\rowcolor[HTML]{DFDFDF} 
Ren \textit{et al.}~\cite{ren2017cyber} & & \multicolumn{1}{c|}{\checkmark} &  &  & \multicolumn{1}{c|}{} & \checkmark & & \checkmark & & & \checkmark & \multicolumn{1}{c|}{}\\
He \textit{et al.}~\cite{he2016security} & & \multicolumn{1}{c|}{\checkmark} &  & \checkmark & \multicolumn{1}{c|}{} & \checkmark & &  & & & \checkmark & \multicolumn{1}{c|}{\checkmark}\\
\rowcolor[HTML]{DFDFDF} 
Wu \textit{et al.}~\cite{wu2018establishment} & \checkmark & \multicolumn{1}{c|}{\checkmark} &  & \checkmark & \multicolumn{1}{c|}{} & & \checkmark & \checkmark & \checkmark & & & \multicolumn{1}{c|}{}\\
Fey \textit{et al.}~\cite{fey20173d} & & \multicolumn{1}{c|}{\checkmark} &  & \checkmark & \multicolumn{1}{c|}{} & & & & \checkmark & & & \multicolumn{1}{c|}{\checkmark}\\
\rowcolor[HTML]{DFDFDF} 
Elhabashy \textit{et al.}~\cite{elhabashy2019cyber} & & \multicolumn{1}{c|}{\checkmark} &  & \checkmark & \multicolumn{1}{c|}{} & & & \checkmark & & & & \multicolumn{1}{c|}{}\\
Slaughter \textit{et al.}~\cite{slaughter2017ensure} & \checkmark & \multicolumn{1}{c|}{\checkmark} &  & \checkmark & \multicolumn{1}{c|}{} & & & \checkmark & & \checkmark & & \multicolumn{1}{c|}{}\\
\rowcolor[HTML]{DFDFDF} 
Satchidanandan \textit{et al.}~\cite{satchidanandan2016secure} & & \multicolumn{1}{c|}{\checkmark} &  & \checkmark & \multicolumn{1}{c|}{} & & & \checkmark & & & & \multicolumn{1}{c|}{}\\
Satchidanandan \textit{et al.}~\cite{satchidanandan2018control} &  & \multicolumn{1}{c|}{\checkmark} &  & \checkmark & \multicolumn{1}{c|}{} & & & \checkmark & & & & \multicolumn{1}{c|}{}\\
\rowcolor[HTML]{DFDFDF} 
\textcolor{red}{Woollaston~\cite{honda}} & \textcolor{red}{\checkmark} & \multicolumn{1}{c|}{} &  & \textcolor{red}{\checkmark} & \multicolumn{1}{c|}{} & \textcolor{red}{\checkmark} & & & & & & \multicolumn{1}{c|}{}\\
\textcolor{red}{INCIBE~\cite{aurora}} & \textcolor{red}{\checkmark} & \multicolumn{1}{c|}{} &  & \textcolor{red}{\checkmark} & \multicolumn{1}{c|}{} & \textcolor{red}{\checkmark} & & & & & & \multicolumn{1}{c|}{}\\
\rowcolor[HTML]{DFDFDF} 
\textcolor{blue}{Satchidanandan \textit{et al.}~\cite{proceedings}} &  & \multicolumn{1}{c|}{\textcolor{blue}{\checkmark}} &  & \textcolor{blue}{\checkmark} & \multicolumn{1}{c|}{} & & & \textcolor{blue}{\checkmark}  & & & & \multicolumn{1}{c|}{}\\
\textcolor{blue}{Behera \textit{et al.}~\cite{behera2019system}} &  & \multicolumn{1}{c|}{\textcolor{blue}{\checkmark}} &  & \textcolor{blue}{\checkmark} & \multicolumn{1}{c|}{} & &  & \textcolor{blue}{\checkmark} & & & & \multicolumn{1}{c|}{}\\

\specialrule{0.8pt}{1pt}{1pt}
\end{tabular}
}
\end{tiny}
\end{table*}

